A Convex Parameterization of Robust Recurrent Neural Networks

Recurrent neural networks (RNNs) are a class of nonlinear dynamical systems often used to model sequence-to-sequence maps. RNNs have excellent expressive power but lack the stability or robustness guarantees that are necessary for many applications. In this paper, we formulate convex sets of RNNs with stability and robustness guarantees. The guarantees are derived using incremental quadratic constraints and can ensure global exponential stability of all solutions, and bounds on incremental $ \ell_2 $ gain (the Lipschitz constant of the learned sequence-to-sequence mapping). Using an implicit model structure, we construct a parametrization of RNNs that is jointly convex in the model parameters and stability certificate. We prove that this model structure includes all previously-proposed convex sets of stable RNNs as special cases, and also includes all stable linear dynamical systems. We illustrate the utility of the proposed model class in the context of non-linear system identification.

==> Discussion.tex <==
\remove{\section{Discussion}
We have focused on the case where $G$ is a linear system and $\Phi$ is described by simple sector bound quadratic constraints, however both of these assumptions can be relaxed with some additional technical considerations.

All of our results can be extended to the case where the nominal system $G$ is a smooth nonlinear state space model. When $G$ is no longer a linear system however, the stability conditions take the form of pointwise LMIs. This allows us to deal with state dependent contraction metrics as $E$ now becomes a state dependent function and the contraction metric takes the form $E(x)^\top P^{-1} E(x)$ \cite{Tobenkin:2017}. For the case where $G$ is a polynomial state space model, sum of squares programming can be used to enforce the LMIs.

The conservatism of the IQC framework is largely associated with the accuracy of the IQC descriptors used for the activation function. For the non-incremental case, extensive libraries of IQC descriptors have been developed, e.g. the Zames-Falb, Popov and RL/RC multipliers. In the incremental case was shown that these descriptors cannot be easily used as they do not preserve incremental positivity \cite{Kulkarni:2002}. To the authors' knowledge, it remains an open problem to to find more expressive IQCs for activation functions that are valid for incremental and differential analysis.}

%It remains an open question as to what dynamic IQC multipliers exist in the incremental/differential case.

